Birational Weyl Group Action on the Symplectic Groupoid and Cluster Algebras

A. Bondal introduced the symplectic groupoid of triangular bilinear forms. This groupoid induces a Poisson structure on $\mathcal A_n$, the space of $n\times n$ unipotent upper-triangular matrices, governed by the classical $\mathfrak{so}(n)$ reflection equation. L. Chekhov and M. Shapiro described log-canonical coordinates on this symplectic groupoid via the $\mathcal A_n$-quiver. We introduce a birational Weyl-group action on the symplectic groupoid, generated by cluster transformations associated with cycles of the quiver. We prove that the matrix entries on $\mathcal A_n$ are invariant under this action. V. Fock and L. Chekhov defined a Poisson map $\phi_n:\mathcal T_{g,s}\to\mathcal A_n$, where $s\in\{1,2\}$. Every $A\in\operatorname{Im}(\phi_n)$ satisfies $\operatorname{rank}(A+A^T)\leq 4$, which provides a natural criterion for a cluster Poisson reduction of $\mathcal A_n$. The corresponding rank-condition locus has several irreducible components. We prove that the Weyl group acts transitively on these components and that the associated reductions are conjugate. Thus, it suffices to determine the reduction on a single component. For even $n$, we show that the longest Weyl-group element corresponds to a cluster Donaldson--Thomas transformation. The resulting theta basis is used to characterize the Weyl-invariant regular-function algebra in terms of the matrix entries on $\mathcal A_n$. In contrast, the $\mathcal A_n$-quiver admits no reddening sequence for odd $n$. Finally, we consider the $\Sigma_n$-quiver, a frozen extension of the $\mathcal A_{n+1}$-quiver used in J. Song's cluster realization of the $\imath$-quantum group of type $\mathrm{AI}_n$. For odd $n$, we identify the image of the classical limit of Song's embedding with a quotient of the corresponding Weyl-invariant Poisson algebra.

==> new..filterlation.tex <==
documentclass[11pt]{article}
\usepackage[margin=1in]{geometry}
\usepackage{amsmath,amssymb,amsthm}
\usepackage[hidelinks]{hyperref}

\newtheorem{theorem}{Theorem}[section]
\newtheorem{proposition}[theorem]{Proposition}
\newtheorem{lemma}[theorem]{Lemma}
\newtheorem{corollary}[theorem]{Corollary}
\newtheorem{conjecture}[theorem]{Conjecture}
\newtheorem{assumption}[theorem]{Assumption}
\newtheorem{question}[theorem]{Open problem}
\theoremstyle{definition}
\newtheorem{definition}[theorem]{Definition}
\theoremstyle{remark}
\newtheorem{remark}[theorem]{Remark}
\newtheorem{warning}[theorem]{Warning}

\newcommand{\C}{\mathbb C}
\newcommand{\Z}{\mathbb Z}
\newcommand{\OO}{\mathcal O}
\newcommand{\X}{\mathcal X_{|\mathcal A_n|}}
\newcommand{\A}{\mathcal A_n}
\newcommand{\W}{W_n}
\newcommand{\parity}{\operatorname{par}}
\newcommand{\Span}{\operatorname{Span}_{\C}}
\newcommand{\val}{\operatorname{val}}
\newcommand{\gr}{\operatorname{gr}}
\newcommand{\Supp}{\operatorname{Supp}}
\newcommand{\Frac}{\operatorname{Frac}}
\newcommand{\Av}{\operatorname{Av}_{\W}}
\newcommand{\ka}{\boldsymbol{k}}
\newcommand{\zero}{\boldsymbol{0}}
\newcommand{\one}{\boldsymbol{1}}
\newcommand{\eps}{\varepsilon}
\newcommand{\m}{\mathfrak m}
\newcommand{\aideal}{\mathfrak a}

\title{Higher Geodesic Classes and a Bifiltered Repair\\of the Weyl-Invariant Generation Argument}
\author{Woojin Choi}
\date{Working note --- rigorous conditional architecture}

\begin{document}
\maketitle

\begin{abstract}
This note records and audits a proposed replacement for the infinite symmetrization step in the proof of the Weyl-invariant generation theorem.  The current manuscript constructs, for each lattice point $l$, a distinguished regular function $h_l$ by choosing the smallest Casimir exponents for which all formal-geodesic exponents are nonnegative.  It then expands a regular function as a generally infinite triangular series in the $h_l$ and groups that series by Weyl-group orbits.  The latter operation is not justified merely by ordinary linear independence, because the componentwise support order used in the expansion is not Weyl-stable.

The repair developed here introduces higher classes $h_l^{\ka}$, indexed by a nonnegative multi-level $\ka$, which parametrize the nonminimal solutions of the same valuation equations.  Increasing $\ka$ increases the formal-geodesic exponents and hence the geodesic-adic order.  Since the Weyl action preserves the full formal-geodesic exponent vector, it preserves the level $\ka$; distinct levels do not mix under the action.  A second, Casimir-augmentation filtration truncates the remaining central directions.  Finite expressions in the resulting quotients can then be symmetrized by Reynolds averaging.

The argument is complete only conditionally.  The higher classes algebraically span the intermediate algebra generated by the formal geodesics and Casimirs, but this does not automatically imply that they span the finite quotients of the full regular-function ring.  A local algebra criterion reducing that spanning problem to a comparison of local rings is formulated.  Even after finite-level spanning is established, an adic closedness statement remains necessary to return from arbitrarily high congruences to actual membership in the geodesic algebra.  Every unproved input is isolated below.
\end{abstract}

\tableofcontents

\section{Ambient rings and manuscript input}

Set
\[
  R:=\OO(\X),
  \qquad
  G:=\OO(\A)\subseteq R.
\]
The algebra $G$ is the unital Poisson algebra generated by the elementary formal geodesic functions; by the Bondal relations it contains all formal geodesic functions $A_{ij}$.
Let
\[
  m:=\left\lfloor\frac n2\right\rfloor,
  \qquad
  N:=\frac{n(n-1)}2.
\]

The proposed argument imports the following statements from the manuscript, or else treats them as explicit assumptions when their hypotheses are not yet known.

\begin{enumerate}
\item The Weyl group $\W$ acts on the relevant regular ring $R$ by algebra automorphisms.  For odd $n$, preservation by the last birational reflection must be verified separately.

\item Every formal geodesic function is fixed:
\[
  w(A_{ij})=A_{ij}
  \qquad(w\in\W).
\]

\item The Weyl action permutes and inverts the Casimirs $K_1,\dots,K_m$.

\item For every $l\in\Z^N$, the manuscript constructs
\[
  h_l
  =\prod_{s=1}^{m}K_s^{q_s^0(l)}
   \prod_{1\le i<j\le n}A_{ij}^{p_{ij}^0(l)},
  \qquad p_{ij}^0(l)\in\Z_{\ge0},
\]
where the Casimir exponents $q_s^0(l)$ are chosen minimally, and $h_l$ has unique minimal Laurent multidegree $l$.

\item The family $\{h_l\}_{l\in\Z^N}$ is permuted by $\W$.  The key point in the manuscript's proof is that the Weyl action preserves the full exponent vector of the formal-geodesic part:
\[
  p_{ij}(w(h))=p_{ij}(h).
\]

\item Weyl-orbit sums of Casimir monomials belong to $G$.  Consequently, whenever a formal-geodesic monomial factors out of a Weyl orbit, the resulting orbit sum belongs to $G$.
\end{enumerate}

\section{The gap in the original infinite symmetrization}

The manuscript obtains a generally infinite triangular expression
\[
  f\sim\sum_l c_lh_l
\]
by repeatedly cancelling minimal Laurent multidegrees.  The relation $\sim$ is not, by itself, an equality in a topological algebra.  In particular, the componentwise order used to organize the elimination is not generally preserved by the Weyl action:
\[
  l\le l'
  \not\Longrightarrow
  w(l)\le w(l').
\]

\begin{warning}
Ordinary linear independence of the $h_l$ proves uniqueness only for finite linear combinations.  It does not justify termwise Weyl action, coefficient comparison, or orbitwise regrouping in an infinite formal family.  A valid proof must either construct a Weyl-stable completion in which the family is topologically summable and unique, or avoid the infinite regrouping altogether.
\end{warning}

The present approach follows the second option: one seeks finite spanning statements in Weyl-stable quotients and averages only finite expressions.

\section{The geodesic degree and the missing central directions}

Write the block decomposition
\[
  B_{\mathrm{deg}}^Tl
  =\begin{bmatrix}
     L_1(l)\\ \vdots\\ L_m(l)
   \end{bmatrix},
  \qquad
  L_i(l)\in\Z^{N_i}.
\]
For each block define normalized range coordinates
\[
  \rho_{i,r}(l)
  :=[L_i(l)]_r-\min_s[L_i(l)]_s.
\]
Thus $\rho_{i,r}(l)\ge0$ and $\min_r\rho_{i,r}(l)=0$.

Let
\[
  d_0(l):=\sum_{i<j}p_{ij}^0(l).
\]
If $n=2m+1$ is odd, then
\begin{equation}\label{eq:odd-d0}
  d_0(l)
  =\sum_{i=1}^{m}\sum_{r=1}^{n}\rho_{i,r}(l).
\end{equation}
If $n=2m$ is even, define
\[
  \eps_m(l)
  :=2\left\lceil
  -\frac{\min_s[L_m(l)]_s}{2}
  \right\rceil
  +\min_s[L_m(l)]_s
  \in\{0,1\}.
\]
Then
\begin{equation}\label{eq:even-d0}
  d_0(l)
  =\sum_{i=1}^{m-1}\sum_{r=1}^{n}\rho_{i,r}(l)
  +\sum_{r=1}^{m}\rho_{m,r}(l)
  +m\eps_m(l).
\end{equation}

\begin{proposition}[Non-properness of the minimal geodesic degree]\label{prop:d0nonproper}
The function $d_0(l)$ controls the spread inside each block $L_i(l)$ but not its constant-vector component.  Hence boundedness of $d_0(l)$ does not, by itself, imply boundedness of $l$.
\end{proposition}

\begin{proof}
For every scalar $c_i$,
\[
 [L_i(l)]_r+c_i
 -\min_s([L_i(l)]_s+c_i)
 =\rho_{i,r}(l).
\]
Thus all terms in \eqref{eq:odd-d0} are invariant under constant-vector shifts.  In the even final block, the parity correction is unchanged by even constant shifts.  Therefore the displayed formulas cannot control such directions.  Identifying exactly which lattice directions occur as constant shifts is a separate linear-algebra calculation, but the formulas already show that $d_0$ alone is not coercive.
\end{proof}

The unmeasured directions are expected to correspond to changes in the Casimir exponents.  This motivates both the higher classes introduced next and a central augmentation filtration.

\section{All nonminimal solutions and the higher classes}

Let
\[
  \delta:=\parity(n)
  =\begin{cases}
  1,&n\text{ odd},\\
  2,&n\text{ even}.
  \end{cases}
\]
For fixed $l$, the manuscript's valuation equations have the block form
\begin{align}
 p_i(l)&=L_i(l)+(q_i-q_{i+1})\one_i,
 &&1\le i<m,\label{eq:block1}\\
 p_m(l)&=L_m(l)+\delta q_m\one_m.\label{eq:blockm}
\end{align}
The distinguished element $h_l=h_l^{\zero}$ uses the minimal integral choices $q_i^0(l)$ for which all entries of the resulting blocks $p_i^0(l)$ are nonnegative.

\subsection{Definition of the higher levels}

For
\[
  \ka=(k_1,\dots,k_m)\in\Z_{\ge0}^m,
\]
define
\begin{equation}\label{eq:qk}
  q_i^{\ka}(l)
  :=q_i^0(l)+\sum_{r=i}^{m}k_r.
\end{equation}
Then
\[
 q_i^{\ka}-q_{i+1}^{\ka}
 =(q_i^0-q_{i+1}^0)+k_i
 \qquad(i<m),
\]
and $q_m^{\ka}=q_m^0+k_m$.  Equations~\eqref{eq:block1}--\eqref{eq:blockm} therefore give
\begin{align}
 p_i^{\ka}(l)&=p_i^0(l)+k_i\one_i,
 &&i<m,\label{eq:pk1}\\
 p_m^{\ka}(l)&=p_m^0(l)+\delta k_m\one_m.\label{eq:pkm}
\end{align}

\begin{definition}[Higher geodesic class]\label{def:higher}
Define
\[
  h_l^{\ka}
  :=\prod_{s=1}^{m}K_s^{q_s^{\ka}(l)}
    \prod_{i<j}A_{ij}^{p_{ij}^{\ka}(l)}.
\]
Then $h_l^{\zero}=h_l$.
\end{definition}

\subsection{Parametrization of all nonminimal solutions}

\begin{proposition}[Normal form for solutions of the valuation equations]\label{prop:normalform}
Fix $l\in\Z^N$.  Assume that $(q,p)$ is an integral solution of \eqref{eq:block1}--\eqref{eq:blockm} with $p\ge0$.  Then there is a unique $\ka\in\Z_{\ge0}^m$ such that
\[
  (q,p)=(q^{\ka}(l),p^{\ka}(l)).
\]
Consequently every monomial $K^qA^p$ with nonnegative formal-geodesic exponents has a unique representation $h_l^{\ka}$, where $l=\val(K^qA^p)$.
\end{proposition}

\begin{proof}
Let
\[
  \Delta q_i:=q_i-q_i^0(l).
\]
Subtracting the minimal solution from \eqref{eq:block1} gives
\[
  p_i-p_i^0(l)
  =(\Delta q_i-\Delta q_{i+1})\one_i
  \qquad(i<m),
\]
and subtracting \eqref{eq:blockm} gives
\[
  p_m-p_m^0(l)=\delta\Delta q_m\one_m.
\]
Set
\[
  k_i:=\Delta q_i-\Delta q_{i+1}
  \quad(i<m),
  \qquad
  k_m:=\Delta q_m.
\]
Because the minimal blocks $p_i^0(l)$ attain the smallest admissible entry---zero for $i<m$, zero in the odd final block, and zero or one in the even final block---the condition $p_i\ge0$ forces $k_i\ge0$.  More explicitly, for $i<m$ one has
\[
  k_i=\min_r p_{i,r},
\]
while in the last block
\[
  k_m=\left\lfloor
  \frac{\min_r p_{m,r}}{\delta}
  \right\rfloor.
\]
Thus $\ka$ is intrinsic and unique.  Telescoping gives
\[
  \Delta q_i=\sum_{r=i}^{m}k_r,
\]
which is exactly \eqref{eq:qk}; equations~\eqref{eq:pk1}--\eqref{eq:pkm} follow.  Finally $l=\val(K^qA^p)$ fixes the lattice index.
\end{proof}

\begin{remark}[Point requiring parity verification]
The proof uses the precise minimal-entry convention in the even last block.  In a manuscript version, the statement that $k_m=\lfloor\min(p_m)/2\rfloor$ should be checked against the parity constraint imposed by the image of $B_{\mathrm{deg}}^T$; the formula is correct once the minimal remainder $\eps_m(l)\in\{0,1\}$ is fixed.
\end{remark}

\section{The intermediate algebra spanned by the higher classes}

Define
\[
  S:=G[K_1^{\pm1},\dots,K_m^{\pm1}]\subseteq R.
\]

\begin{corollary}[Algebraic spanning of $S$]\label{cor:Sspan}
The higher classes span $S$ as a complex vector space:
\[
  S
  =\Span\{h_l^{\ka}:l\in\Z^N,
          \ka\in\Z_{\ge0}^m\}.
\]
Every element of $S$ has a finite expression in these classes.
\end{corollary}

\begin{proof}
Every element of $S$ is a finite linear combination of monomials $K^qA^p$ with $p\ge0$.  Proposition~\ref{prop:normalform} identifies each such monomial with a unique $h_l^{\ka}$.
\end{proof}

\begin{warning}
Corollary~\ref{cor:Sspan} concerns $S$, not the full regular ring $R$.  It does not imply that the higher classes span $R$, or even that their images span an arbitrary quotient of $R$.  The passage from $S$ to $R$ is a separate local-generation problem.
\end{warning}

\section{Weyl stability of the higher levels}

\begin{proposition}[Level preservation]\label{prop:levelpreservation}
Assume that the Weyl action preserves the entire formal-geodesic exponent vector $p$.  Then for every $w\in\W$, $l\in\Z^N$, and $\ka\in\Z_{\ge0}^m$, there exists a unique lattice point $w\star_{\ka}l$ such that
\[
  w(h_l^{\ka})=h_{w\star_{\ka}l}^{\ka}.
\]
In particular, for fixed $\ka$ the family
\[
  \mathcal H_{\ka}:=
  \{h_l^{\ka}:l\in\Z^N\}
\]
is $\W$-stable, and distinct $\ka$-levels do not mix.
\end{proposition}

\begin{proof}
Write
\[
  w(h_l^{\ka})=K^{q'}A^{p'}.
\]
By hypothesis $p'=p^{\ka}(l)$.  The level $\ka$ is recovered intrinsically from $p'$ by the block-minimum formulas in the proof of Proposition~\ref{prop:normalform}.  Hence the image has the same level $\ka$.  Its unique Laurent minimal multidegree defines $w\star_{\ka}l$, and uniqueness follows from the normal form.
\end{proof}

\begin{corollary}[Orbit-sum factorization]\label{cor:orbitsum}
For fixed $l$ and $\ka$, the formal-geodesic monomial is constant along the Weyl orbit.  Hence
\[
  (h_l^{\ka})^{\W}
  =A^{p^{\ka}(l)}
   \sum_{q'\in\W\cdot q^{\ka}(l)}K^{q'}.
\]
If Weyl-orbit sums of Casimir monomials belong to $G$, then
\[
  (h_l^{\ka})^{\W}\in G.
\]
\end{corollary}

\section{Geodesic-order growth in the higher direction}

Let
\[
  I:=(A_{ij}:i<j)_R.
\]
Define
\[
  d(l,\ka):=\sum_{i<j}p_{ij}^{\ka}(l).
\]
Equations~\eqref{eq:pk1}--\eqref{eq:pkm} yield
\begin{equation}\label{eq:degreegrowth}
 d(l,\ka)
 =d_0(l)
 +\sum_{i=1}^{m-1}N_i k_i
 +N_m\delta k_m.
\end{equation}

\begin{proposition}[Higher levels vanish geodesic-adically]\label{prop:vanish}
For every $l$ and $\ka$,
\[
  h_l^{\ka}\in I^{d(l,\ka)}.
\]
For fixed $a$ and $l$, only finitely many $\ka$ satisfy $d(l,\ka)<a$.  Thus $h_l^{\ka}\in I^a$ for all sufficiently large levels $\ka$.
\end{proposition}

\begin{proof}
The first assertion follows because $h_l^{\ka}$ contains exactly $d(l,\ka)$ formal-geodesic factors, counted with multiplicity.  Formula~\eqref{eq:degreegrowth} has strictly positive coefficients in every $k_i$, so its sublevel sets in $\Z_{\ge0}^m$ are finite.
\end{proof}

\begin{remark}
This is the decisive difference between $h_l^{\ka}$ and a bare sequence $K^qA^p$ with fixed $p$.  The latter does not converge to zero in the Casimir-augmentation topology as $|q|\to\infty$, whereas increasing $\ka$ forces the geodesic exponent vector itself to grow.
\end{remark}

\section{The central augmentation and the combined ideal}

A base point on the Casimir torus must be chosen compatibly with the characteristic-polynomial relations.  Let
\[
  \kappa\in\{1,-1\}
\]
denote the chosen Weyl-fixed central value.  The natural value is to be verified from the actual fiber; the factorization in the manuscript suggests that the parity convention may matter.

Define in $S$
\[
  \aideal
  :=(A_{ij},K_1-\kappa,\dots,K_m-\kappa)_S.
\]
Define in $R$
\[
  J_\kappa
  :=(K_1-\kappa,\dots,K_m-\kappa)_R,
\]
and set
\begin{equation}\label{eq:H}
  H:=\aideal R=I+J_\kappa.
\end{equation}

\begin{lemma}[Weyl stability of $H$]\label{lem:Hstable}
Assume that the Weyl group permutes and inverts the Casimirs and that $\kappa^2=1$.  Then $I$, $J_\kappa$, and $H$ are $\W$-stable.
\end{lemma}

\begin{proof}
The stability of $I$ follows from $w(A_{ij})=A_{ij}$.  A permutation sends $K_i-\kappa$ to $K_j-\kappa$.  An inversion gives
\[
  K_j^{-1}-\kappa
  =-\kappa K_j^{-1}(K_j-\kappa),
\]
which belongs to $J_\kappa$.  Thus $J_\kappa$ is stable, and so is their sum $H$.
\end{proof}

\subsection{Bifiltration versus $H$-adic filtration}

\begin{proposition}[Cofinality]\label{prop:cofinal}
The bifiltration $\{I^a+J_\kappa^b\}_{a,b\ge1}$ and the $H$-adic filtration $\{H^N\}_{N\ge1}$ are cofinal.  More precisely,
\[
  H^{a+b-1}\subseteq I^a+J_\kappa^b,
  \qquad
  I^N+J_\kappa^N\subseteq H^N.
\]
Consequently
\[
  \bigcap_{a,b\ge1}
  (G+I^a+J_\kappa^b)
  =\bigcap_{N\ge1}(G+H^N).
\]
\end{proposition}

\begin{proof}
Every summand $I^rJ_\kappa^s$ in the binomial expansion of $H^{a+b-1}$ satisfies $r\ge a$ or $s\ge b$.  The second inclusion is immediate from $I,J_\kappa\subseteq H$.
\end{proof}

\section{What is finite in the combined quotients}

Let
\[
  C_K:=\C[K_1^{\pm1},\dots,K_m^{\pm1}],
  \qquad
  \m_\kappa:=(K_1-\kappa,\dots,K_m-\kappa).
\]
For every $b$, the quotient $C_K/\m_\kappa^b$ is finite-dimensional; Laurent powers admit truncated binomial expansions around $K_i=\kappa$.

Combining this with Proposition~\ref{prop:vanish} gives a genuine finite-data statement: modulo $I^a+J_\kappa^b$, only finitely many formal-geodesic exponent patterns of total size $<a$, finitely many $\ka$-levels for each minimal pattern, and finitely many truncated central monomials are visible.

\begin{warning}[Finite data is not yet spanning]\label{warn:notspan}
This finite-data statement shows that the images of all higher classes span a finite-dimensional subspace of $R/(I^a+J_\kappa^b)$.  It does not prove that this subspace is the entire quotient.  The higher classes span $S$ algebraically, but a separate argument is required to compare $S$ and $R$ near the chosen fiber.
\end{warning}

\section{A local algebra criterion for finite-level spanning}

The natural morphism of affine schemes is
\[
  \pi:\operatorname{Spec}R\longrightarrow\operatorname{Spec}S.
\]
Let $\aideal\subset S$ be as above and $H=\aideal R$.

\begin{assumption}[Local comparison hypotheses]\label{ass:local}
Assume:
\begin{enumerate}
\item $\aideal$ is maximal and $S/\aideal\simeq\C$;
\item $H$ is maximal and $R/H\simeq\C$;
\item $R_H$ is finite as an $S_{\aideal}$-module;
\item the natural local map $S_{\aideal}\to R_H$ is injective.
\end{enumerate}
\end{assumption}

\begin{warning}[Localization notation]
The notation $R_H$ is legitimate only after $H$ has been shown prime, in particular maximal under (L2).  If $H$ is merely proper, one must instead choose a maximal ideal $\mathfrak q\supseteq H$ and work with $R_{\mathfrak q}$.
\end{warning}

\begin{proposition}[Local equality via Nakayama]\label{prop:localequality}
Under Assumption~\ref{ass:local},
\[
  R_H=S_{\aideal}.
\]
\end{proposition}

\begin{proof}
Let
\[
  M:=R_H/S_{\aideal}.
\]
By (L3), $M$ is a finite $S_{\aideal}$-module.  The residue-field assumptions imply that the map
\[
  S_{\aideal}/\aideal S_{\aideal}
  \longrightarrow
  R_H/\aideal R_H
\]
is surjective, with both sides isomorphic to $\C$.  Therefore
\[
  M/\aideal M=0.
\]
Nakayama's lemma gives $M=0$.
\end{proof}

\begin{proposition}[Finite-level spanning under local equality]\label{prop:finitelevelspan}
Under Assumption~\ref{ass:local}, for every $N\ge1$ the natural image of $S$ spans the localization of $R/H^N$ at the point $H$.  If, in addition, $H$ is the only prime of $R$ over $\aideal$ that contributes to $R/H^N$, then
\[
  R/H^N=\operatorname{im}(S\to R/H^N).
\]
Consequently,
\[
  R/H^N
  =\Span\{[h_l^{\ka}]_N:
    l\in\Z^N,\ \ka\in\Z_{\ge0}^m\}.
\]
\end{proposition}

\begin{proof}
The local equality gives surjectivity after localizing at $H$.  To deduce global surjectivity on the $H$-supported quotient, one must know that no other support remains; this is the additional hypothesis in the statement.  Once the image of $S$ is all of $R/H^N$, Corollary~\ref{cor:Sspan} gives the final equality.
\end{proof}

\begin{warning}[Why the support hypothesis is explicit]
The equality $R_H=S_{\aideal}$ is local at one point.  It does not automatically imply that $S\to R/H^N$ is globally surjective if the scheme defined by $H$ has additional support or if localization kills a nonzero cokernel.  A clean sufficient condition is that $H$ be maximal and $R/H^N$ be supported only at $H$.
\end{warning}

\section{Finite-level Weyl averaging}

Assume henceforth that finite-level spanning holds, either through Proposition~\ref{prop:finitelevelspan} or by a direct elimination theorem.

\begin{proposition}[Invariant approximation]\label{prop:average}
Let $f\in R^{\W}$.  For every $N\ge1$, there exists $g_N\in G$ such that
\[
  f-g_N\in H^N.
\]
Equivalently,
\[
  f\in G+H^N
  \qquad\text{for every }N.
\]
\end{proposition}

\begin{proof}
By finite-level spanning, choose a finite expression
\[
  [f]_N
  =\sum_{(l,\ka)\in F_N}
    c_{l,\ka}[h_l^{\ka}]_N.
\]
Because $H$ is Weyl-stable, $R/H^N$ is a finite-dimensional or at least algebraic $\W$-representation on the finite span in question.  Since $[f]_N$ is invariant,
\begin{align*}
 [f]_N
 &=\frac1{|\W|}\sum_{w\in\W}w([f]_N)\\
 &=\frac1{|\W|}
   \sum_{(l,\ka)\in F_N}c_{l,\ka}
   \sum_{w\in\W}[w(h_l^{\ka})]_N.
\end{align*}
By Proposition~\ref{prop:levelpreservation}, the inner sum stays in the same $\ka$-level.  By Corollary~\ref{cor:orbitsum}, it is represented by an element of $G$.  Hence the entire class is represented by some $g_N\in G$.
\end{proof}

\section{The final closedness problem}

Finite-level averaging gives
\[
  f\in\bigcap_{N\ge1}(G+H^N).
\]
To conclude $f\in G$, one needs the following independent statement.

\begin{assumption}[$H$-adic closedness of $G$]\label{ass:closed}
\begin{equation}\label{eq:closedness}
  \bigcap_{N\ge1}(G+H^N)=G.
\end{equation}
Equivalently,
\[
  \bigcap_{N\ge1}\frac{G+H^N}{G}=0
  \quad\text{inside the vector space }R/G.
\]
\end{assumption}

\begin{warning}
Since $G$ is generally not an ideal of $R$, $R/G$ is not naturally an $R$-module.  One should formulate closedness using the subspaces $(G+H^N)/G$, not by writing $H^N(R/G)$ without additional justification.
\end{warning}

\begin{theorem}[Conditional repaired invariant-generation theorem]\label{thm:main}
Assume:
\begin{enumerate}
\item $\W$ acts on $R$ by algebra automorphisms;
\item the higher-class normal form of Proposition~\ref{prop:normalform} holds;
\item finite-level spanning of $R/H^N$ by the $h_l^{\ka}$ holds for every $N$;
\item Weyl-orbit sums of Casimir monomials belong to $G$;
\item $G$ is $H$-adically closed in $R$.
\end{enumerate}
Then
\[
  R^{\W}\subseteq G.
\]
\end{theorem}

\begin{proof}
For $f\in R^{\W}$, Proposition~\ref{prop:average} gives $f\in G+H^N$ for every $N$.  Assumption~\ref{ass:closed} then gives $f\in G$.
\end{proof}

\section{Possible routes to closedness}

\subsection{A compatible scalar grading}
A bounded-below scalar grading on $R/G$ for which membership in $(G+H^N)/G$ forces degree at least $cN-C$ would prove \eqref{eq:closedness}.  The original vector-valued multidegree is not enough unless it is converted into a proper scalar height compatible with multiplication by both geodesic and central augmentation generators.

\subsection{A direct valuation estimate}
It suffices to construct a function $\delta$ on nonzero classes of $R/G$ such that
\[
  0\ne\xi\in(G+H^N)/G
  \Longrightarrow
  \delta(\xi)\ge cN-C,
\]
with $c>0$, while every fixed class has finite $\delta$.

\subsection{Module-finiteness with additional hypotheses}
If $R$ is finite as a $G$-module, then $R/G$ is finite over $G$.  This is useful but does not by itself prove separation for an arbitrary filtration.  A local Jacobson-radical condition, a compatible grading, or an Artin--Rees setup for an ideal extended from $G$ would still be needed.  Generic finiteness of
\[
  \Frac(R)/\Frac(G)
\]
does not imply module-finiteness.

\subsection{Direct extremal-term algebraization}
One may instead prove that an infinite family of nonzero orbit contributions cannot represent a finite Laurent polynomial.  This requires distinguished noncancellable extremal monomials for the higher orbit sums and a rigorous comparison between the $H$-adic topology and coefficientwise Laurent convergence.

\section{Precise status of the program}

\subsection*{Established within this note, conditional only on manuscript inputs}
\begin{enumerate}
\item The formula for the minimal geodesic degree is non-coercive in central directions.
\item The higher classes $h_l^{\ka}$ parameterize all nonminimal solutions of the valuation equations, subject to the stated parity convention.
\item The higher classes algebraically span $S=G[K_1^{\pm1},\dots,K_m^{\pm1}]$.
\item The Weyl action preserves each level $\ka$ because it preserves $p$.
\item The geodesic-adic order grows linearly with $\ka$.
\item The combined ideal satisfies $H=\aideal R=I+J_\kappa$.
\item The bifiltration and $H$-adic filtration are cofinal.
\item Finite-level spanning plus orbit-sum generation implies invariant approximation modulo every $H^N$.
\item Closedness then implies $R^{\W}\subseteq G$.
\end{enumerate}

\subsection*{Remaining mathematical inputs}
\begin{enumerate}
\item Verify the parity-correct central value $\kappa$ and prove that $H$ is proper; ideally determine $R/H$ scheme-theoretically.
\item Prove the local comparison hypotheses, or find a direct finite-level elimination proving
\[
  R/H^N
  =\Span\{[h_l^{\ka}]_N\}
  \quad\text{for every }N.
\]
\item Prove the closedness identity \eqref{eq:closedness}, or replace it by a direct algebraization theorem.
\item Recheck that the Casimir orbit-sum result is independent of the flawed infinite symmetrization argument.
\item Treat the square-root and frozen-extension settings separately; the current proof cannot be transferred by analogy without new ideals, normal forms, spanning, and closedness statements.
\end{enumerate}

\section{Suggested proof order}

A disciplined proof attempt should proceed in the following order.

\begin{enumerate}
\item Prove Proposition~\ref{prop:normalform} directly from the matrix equations, including the even parity case.
\item Prove level preservation from $p$-preservation.
\item Determine the correct central base point $\kappa$ and calculate $R/H$.
\item Prove finite-level spanning, preferably first for $R/H$ and $R/H^2$, then formulate the general induction or local-algebra theorem.
\item Only after spanning is complete, use Reynolds averaging.
\item Finally attack closedness.  Do not regard congruence modulo every $H^N$ as equality in $G$ until this final step is proved.
\end{enumerate}

\section{Conclusion}

The higher classes $h_l^{\ka}$ resolve a genuine defect in the original basis candidate: the minimal classes $h_l$ record only the smallest nonnegative formal-geodesic exponents, while the nonminimal solutions of the same valuation equations form additional levels.  These levels are particularly well suited to Weyl symmetrization because the Weyl action preserves $p$, and therefore preserves $\ka$.  Their geodesic order grows with $\ka$, so high levels vanish in finite geodesic quotients.

This does not by itself finish the invariant-generation theorem.  The higher classes span the intermediate algebra $S$, whereas the theorem concerns the full ring $R$.  The remaining bridge is finite-level spanning of $R/H^N$, obtainable either from a direct finite elimination or from a sufficiently strong local comparison between $S$ and $R$.  Once that bridge is established, the only final obstruction is the closedness of $G$ in the $H$-adic topology.  The resulting architecture is therefore mathematically coherent, but it remains a conditional research program rather than a completed repair.

\end{document}

